Sample Design Engineering: An Empirical Study of What Makes Good Downstream Fine-Tuning Samples for LLMs

In the burgeoning field of Large Language Models (LLMs) like ChatGPT and LLaMA, Prompt Engineering (PE) is renowned for boosting zero-shot or in-context learning (ICL) through prompt modifications. Yet, the realm of the sample design for downstream fine-tuning, crucial for task-specific LLM adaptation, is largely unexplored. This paper introduces Sample Design Engineering (SDE), a methodical approach to enhancing LLMs' post-tuning performance by refining input, output, and reasoning designs. We conduct a series of in-domain (ID) and out-of-domain (OOD) experiments to assess the impact of various design options on LLMs' downstream performance, revealing several intriguing patterns that hold consistently across different LLMs. Based on these insights, we propose an integrated SDE strategy, combining the most effective options, and validate its consistent superiority over heuristic sample designs in complex downstream tasks like multi-aspect sentiment analysis, event extraction, and nested entity recognition. Additionally, analyses of LLMs' inherent prompt/output perplexity, zero-shot, and ICL abilities illustrate that good PE strategies may not always translate to good SDE strategies. Code available at https://github.com/beyondguo/LLM-Tuning.

==> tables/Exp-Chat-main.tex <==
% 1. 添加下面这部分到表格中，为了节省空间：
% \small
% \centering
% \setlength\tabcolsep{2pt}
% 2. 将 `\%` 都统一去除，节省空间
% 3. 将各个model的Chat或者Base，写成下标
% 4. ID-avg, OOD-avg 替换成 avg

\begin{table*}[]
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{cccccccc|cccccc} 
\toprule
\multicolumn{2}{l}{\textbf{In-Domain Tasks}}  & \multicolumn{6}{c|}{Sentiment Analysis  Performace (Kappa ↑)}                                                                            & \multicolumn{6}{c}{Format Adherence  Performance (Error Rate ↓)}                                                                        \\ \toprule
\multicolumn{1}{l}{}                                                      & \multicolumn{1}{l}{} & \multicolumn{2}{c}{InternLM$_{Chat}$}           & \multicolumn{2}{c}{Baichuan2$_{Chat}$}          & \multicolumn{2}{c}{Alpaca2$_{Chat}$}             & \multicolumn{2}{c}{InternLM$_{Chat}$}           & \multicolumn{2}{c}{Baichuan2$_{Chat}$}          & \multicolumn{2}{c}{Alpaca$_{Chat}$}             \\ 
\multicolumn{1}{l}{}                                                      & \multicolumn{1}{l}{} & avg               & rank                 & avg               & rank                 & avg               & rank                 & avg               & rank                 & avg               & rank                 & avg               & rank                 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ Designs\end{tabular}}  &  ins-last  & 74.21              & 3                    & 75.87              & 2                    & 76.83              & 1                    & 0.00               & 1                    & 0.03               & 2                    & 0.00               & 1                    \\ 
                                                                          & ins-first            & 76.49              & 1                    & 76.19              & 1                    & 76.63              & 2                    & 0.01               & 2                    & 0.27               & 4                    & 0.00               & 1                    \\ 
                                                                          & text2label           & 74.75              & 2                    & 68.19              & 4                    & 74.62              & 3                    & 0.08               & 4                    & 0.08               & 3                    & 0.06               & 4                    \\ 
                                                                          & modeling input       & 70.38              & 4                    & 72.25              & 3                    & 74.07              & 4                    & 0.01               & 2                    & 0.00               & 1                    & 0.00               & 1                    \\ 
                                                                          \midrule
                                                                          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\ 
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Output\\ Designs\end{tabular}} & natural-concat       & 74.21              & 3                    & 75.87              & 2                    & 75.85              & 4                    & 0.00               & 1                    & 0.03               & 3                    & 0.00               & 1                    \\ 
                                                                          & digital-label        & 74.23              & 2                    & 75.42              & 4                    & 71.14              & 5                    & 0.00               & 1                    & 0.17               & 1                    & 0.03               & 5                    \\ 
                                                                          & mentioned-only       & 71.89              & 5                    & 72.64              & 5                    & 76.49              & 3                    & 0.00               & 1                    & 0.16               & 2                    & 0.00               & 1                    \\ 
                                                                          & lines-output         & 74.29              & 1                    & 75.80              & 3                    & 76.89              & 1                    & 0.01               & 5                    & 0.00               & 4                    & 0.00               & 1                    \\ 
                                                                          & dict\_output         & 73.35              & 4                    & 75.91              & 1                    & 76.72              & 2                    & 0.00               & 1                    & 0.00               & 4                    & 0.00               & 1                    \\ 
                                                                          \midrule
                                                                          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\ 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CoT\\ Designs\end{tabular}}    & no-CoT               & 73.35              & 3                    & 75.91              & 1                    & 75.97              & 3                    & 0.00               & 1                    & 0.00               & 3                    & 0.00               & 1                    \\ 
                                                                          & CoT                  & 74.74              & 1                    & 75.11              & 3                    & 76.11              & 2                    & 0.27               & 2                    & 15.47              & 1                    & 0.52               & 3                    \\ 
                                                                          & rev-CoT              & 73.76              & 2                    & 75.24              & 2                    & 76.76              & 1                    & 0.34               & 3                    & 0.66               & 2                    & 0.48               & 2                    \\ \midrule 
\multicolumn{1}{l}{}                                                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 

\multicolumn{2}{l}{\textbf{Out-Domain Tasks}}                                                           & \multicolumn{6}{c}{Sentiment Analysis Performace (Kappa ↑)}                                                                             & \multicolumn{6}{c}{Format Adherence Performance (Error Rate ↓)}                                                                         \\ 
\multicolumn{1}{l}{}                                                      & \multicolumn{1}{l}{} & \multicolumn{2}{c}{InternLM$_{Chat}$}           & \multicolumn{2}{c}{Baichuan2$_{Chat}$}          & \multicolumn{2}{c}{Alpaca2$_{Chat}$}             & \multicolumn{2}{c}{InternLM$_{Chat}$}           & \multicolumn{2}{c}{Baichuan2$_{Chat}$}          & \multicolumn{2}{c}{Alpaca$_{Chat}$}             \\ 
\multicolumn{1}{l}{}                                                      & \multicolumn{1}{l}{} & avg              & rank                 & avg              & rank                 & avg              & rank                 & avg              & rank                 & avg              & rank                 & avg              & rank                 \\ 
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ Designs\end{tabular}}  &  ins-last  & 56.56              & 2                    & 55.37              & 2                    & 64.15              & 1                    & 0.00               & 1                    & 0.19               & 2                    & 0.02               & 1                    \\ 
                                                                          & ins-first            & 59.92              & 1                    & 57.60              & 1                    & 63.74              & 2                    & 1.66               & 3                    & 0.99               & 1                    & 0.04               & 2                    \\ 
                                                                          & text2label           & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     & \textbackslash{}     \\ 
                                                                          & modeling input       & 49.26              & 3                    & 49.18              & 3                    & 51.39              & 3                    & 0.23               & 2                    & 0.06               & 3                    & 4.57               & 3                    \\ 
                                                                          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\ 
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Output\\ Designs\end{tabular}} & natural-concat       & 56.56              & 3                    & 55.37              & 3                    & 63.30              & 3                    & 0.00               & 1                    & 0.19               & 2                    & 0.02               & 3                    \\ 
                                                                          & digital-label        & 58.40              & 1                    & 53.70              & 4                    & 55.25              & 5                    & 0.04               & 4                    & 0.12               & 3                    & 4.80               & 5                    \\ 
                                                                          & mentioned-only       & 55.34              & 5                    & 49.99              & 5                    & 61.29              & 4                    & 0.21               & 5                    & 0.30               & 1                    & 3.10               & 4                    \\ 
                                                                          & lines-output         & 57.68              & 2                    & 55.39              & 2                    & 65.06              & 1                    & 0.01               & 3                    & 0.02               & 4                    & 0.00               & 1                    \\ 
                                                                          & dict\_output         & 56.54              & 4                    & 57.80              & 1                    & 64.60              & 2                    & 0.00               & 1                    & 0.01               & 5                    & 0.00               & 1                    \\ 
                                                                          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\ 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CoT\\ Designs\end{tabular}}    & no-CoT               & 56.54              & 2                    & 57.80              & 3                    & 63.28              & 2                    & 0.00               & 1                    & 0.01               & 3                    & 0.00               & 1                    \\ 
                                                                          & CoT                  & 61.44              & 1                    & 59.84              & 1                    & 63.33              & 1                    & 0.89               & 3                    & 16.33              & 1                    & 1.78               & 3                    \\ 
                                                                          & rev-CoT              & 55.95              & 3                    & 58.97              & 2                    & 63.09              & 3                    & 0.38               & 2                    & 1.58               & 2                    & 1.19               & 2                   
 \\ \end{tabular}
\end{table*}

==> tables/Format_Error_Rate.tex <==
% Table generated by Excel2LaTeX from sheet '__'
\begin{table*}
\small
\centering
\setlength\tabcolsep{2pt}
    \begin{tabular}{lcccccc}
    \toprule
          & \multicolumn{3}{c}{\textbf{ID}} & \multicolumn{3}{c}{\textbf{OOD}} \\
          & \textbf{InternLM-Chat} & \textbf{Baichuan2-Chat} & \textbf{LLaMA2-Chat} & \textbf{InternLM-Chat} & \textbf{Baichuan2-Chat} & \textbf{LLaMA2-Chat} \\
    \midrule
    Ins-last & \textbf{0.00 (1)} & 0.05 (2) & \textbf{0.00 (1)} & \textbf{0.07 (1)} & 0.19 (2) & \textbf{0.03 (1)} \\
    Ins-first & 0.04 (3) & 0.35 (4) & \textbf{0.00 (1)} & 1.99 (2) & 2.49 (3) & 0.15 (2) \\
    T2L   & 0.11 (4) & 0.23 (3) & 0.13 (4) & \textbackslash{} & \textbackslash{} & \textbackslash{} \\
    MI    & \textbf{0.00 (1)} & \textbf{0.00 (1)} & 0.01 (3) & 2.48 (3) & \textbf{0.13 (1)} & 6.77 (3) \\
    \midrule
    Natural & \textbf{0.00 (1)} & 0.05 (3) & \textbf{0.00 (1)} & 0.07 (3) & 0.19 (4) & 0.03 (3) \\
    Lines & 0.01 (4) & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.01 (1)} & 0.06 (2) & \textbf{0.00 (1)} \\
    Dict  & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.01 (1)} & \textbf{0.01 (1)} & \textbf{0.00 (1)} \\
    Numerical & \textbf{0.00 (1)} & 0.06 (4) & 0.03 (5) & 0.16 (5) & 0.18 (3) & 7.91 (5) \\
    MO    & 0.01 (4) & 0.52 (5) & \textbf{0.00 (1)} & 0.14 (4) & 0.43 (5) & 0.55 (4) \\
    \midrule
    No-CoT & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.01 (1)} & \textbf{0.01 (1)} & \textbf{0.00 (1)} \\
    CoT   & 0.39 (2) & 27.59 (3) & 0.76 (2) & 0.95 (3) & 25.49 (3) & 2.00 (2) \\
    Rev-CoT & 0.42 (3) & 1.46 (2) & 0.99 (3) & 0.60 (2) & 5.29 (2) & 2.53 (3) \\
    \midrule
          &       &       &       &       &       &  \\
          & \textbf{InternLM-Base} & \textbf{Baichuan2-Base} & \textbf{LLaMA2-Base} & \textbf{InternLM-Base} & \textbf{Baichuan2-Base} & \textbf{LLaMA2-Base} \\
    \midrule
    Ins-last & \textbf{0.01 (1)} & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.01 (1)} & 0.93 (2) & \textbf{0.65 (2)} \\
    Ins-first & 0.07 (3) & 0.06 (3) & \textbf{0.00 (1)} & 1.50 (2) & \textbf{0.45 (1)} & 0.23 (1) \\
    T2L   & 0.11 (4) & 36.47 (4) & 0.01 (3) & \textbackslash{} & \textbackslash{} & \textbackslash{} \\
    MI    & \textbf{0.01 (1)} & 0.01 (2) & 0.01 (4) & 4.26 (3) & 3.91 (3) & 0.74 (3) \\
    \midrule
    Natural & 0.01 (2) & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.01 (1)} & 0.93 (5) & 0.65 (3) \\
    Lines & 0.01 (3) & \textbf{0.00 (1)} & \textbf{0.00 (1)} & 0.03 (2) & \textbf{0.01 (1)} & 0.12 (2) \\
    Dict  & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.00 (1)} & 0.53 (4) & 0.17 (2) & \textbf{0.00 (1)} \\
    Numerical & 0.11 (5) & 0.48 (5) & 0.09 (5) & 0.70 (5) & 0.92 (4) & 2.40 (5) \\
    MO    & 0.03 (4) & 0.00 (1) & 0.02 (4) & 0.34 (3) & 0.35 (3) & 1.93 (4) \\
    \midrule
    No-CoT & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.00 (1)} & \textbf{0.53 (1)} & 0.17 (2) & \textbf{0.00 (1)} \\
    CoT   & 0.56 (2) & 0.58 (2) & 1.04 (3) & 15.04 (2) & \textbf{0.13 (1)} & 1.63 (3) \\
    Rev-CoT & 1.19 (3) & 2.05 (3) & 0.62 (2) & 10.68 (3) & 1.98 (3) & 11.98 (2) \\
    \bottomrule
    \end{tabular}%
    \caption{Format Adherence Performances (Error Rate \%) of Different Data Designs across Various LLMs and Tasks.}
    \label{fig:format-error-rate}
  \label{tab:addlabel}%
\end{table*}%


==> tables/Internlm-Chat_result1.tex <==
\begin{table}[]
\begin{tabular}{ll|cccc|cccc}
\toprule[1.2pt]
   \multicolumn{2}{c|}{\textbf{InternLM-Chat}} &\multicolumn{4}{c|}{\textbf{Kappa}} &\multicolumn{4}{c}{\textbf{\# Wrong format}}  \\
%\cline{3-10}
  \multicolumn{2}{c|}{\textbf{train\_size=500}} & D1 & D2 & D1→D2 & D2→D1  & D1 & D2 & D1→D2 & D2→D1    \\
\hline
  {\color[HTML]{F5222D} Input}&Ins-last & 77.74\%  & 62.78\% & 39.47\%    & 67.07\%   & 0  & 0 & 0 &11\\
  & Ins-first & 80.35\% & 66.09\% &39.49\% &70.90\% & 4 &2 & 13 & 304\\ 
  & T2L & 78.62\%  & 59.63\% & \textbackslash{}& \textbackslash{} &10 &7  & \textbackslash{} & \textbackslash{}\\ 
  & MI& 74.63\% & 51.78\%  & 31.53\% & 53.63\% &0  & 0 & 0 & 395 \\ 
\hline
  {\color[HTML]{F5222D} Output}&Natural & 77.74\%  & 62.78\% & 39.47\%    & 67.07\%   & 0  & 0 & 0 &11\\
  &Lines   & \textbf{78.27\%} & 62.61\% & 40.32\% & 67.99\% & 0 & 1 & 1  & 1  \\
  &Dict   & 77.13\%  & 59.66\% & 39.65\% & 61.29\% & 0 & 0 & 0  & 2  \\
  &Numerical  & 77.65\%  & 62.61\% & 41.65\% & 69.26\% & 0 & 0 & 3  & 23 \\
  &MO & 75.20\%  & 48.88\% & 40.29\% & 62.21\% & 0 & 1 & 16 & 7 \\
\hline
  {\color[HTML]{F5222D}CoT} & No-CoT& 77.13\% & 59.66\% & 39.65\% & 61.29\% & 0  & 0  & 0  & 2   \\
  & CoT  & 76.66\% & 64.01\% & 48.43\% & 67.97\% & 43 & 19 & 30 & 121 \\
  & Rev-CoT  & 77.64\% & 61.24\% & 38.92\% & 66.48\% & 44 & 23 & 23 & 72 \\
  
\midrule[1.2pt]
  \multicolumn{2}{c|}{\textbf{InternLM-Chat}} &\multicolumn{4}{c|}{\textbf{Kappa}} &\multicolumn{4}{c}{\textbf{\# Wrong format}}  \\
  \multicolumn{2}{c|}{\textbf{train\_size=1000}} & D1 & D2 & D1→D2 & D2→D1  & D1 & D2 & D1→D2 & D2→D1    \\
\hline
  {\color[HTML]{F5222D} Input}& Ins-last& 80.49\% & 67.93\% & 43.30\% & 69.82\% & 0  & 0 & 0 & 0 \\
  &Ins-first & 81.73\% & 71.25\% & 46.40\% & 73.43\%  & 0  & 1 & 6  & 259\\
  &T2L & 81.39\% & 68.11\% & \textbackslash{} & \textbackslash{} & 8  & 5 & \textbackslash{} & \textbackslash{} \\
  &MI  & 78.19\% & 62.56\% & 33.32\% & 65.20\%  & 1  & 0 & 8 & 29  \\
\hline
  {\color[HTML]{F5222D} Output}& Natural & 80.49\% & 67.93\% & 43.30\% & 69.82\% & 0  & 0 & 0 & 0 \\
  &Lines & 80.60\% & 67.97\% & 44.98\%& 70.38\%   & 0  & 1 & 0  & 1  \\
  &Dict  & 80.21\% &66.49\% & 46.61\%   & 66.47\%    & 0  & 0 & 0   & 0 \\
  &Numerical & 80.81\% & 67.64\% & 43.93\% & 72.86\% & 0  & 0 & 3  & 3  \\ 
  &MO & 80.08\% & 63.69\% & 43.74\% & 66.94\% & 0  & 0 & 33  & 1 \\
\hline
  {\color[HTML]{F5222D} CoT}& No-CoT  & 80.21\% & 66.49\% & 46.61\% & 66.47\%  & 0  & 0 & 0 & 0 \\
  & CoT & 79.81\% & 69.66\% & 51.90\% & 70.98\% & 36 & 7 & 10 & 132 \\
  &Rev-CoT  & 80.43\% & 67.09\% & 39.94\% & 71.95\%  & 50 & 4 & 19 & 42\\ 
\bottomrule

\end{tabular}
\end{table}

==> tables/mentioned-only_1000.tex <==
%-- coding: UTF-8 --
%\usepackage{CJKutf8}
%\begin{CJK*}{UTF8}{gbsn}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\usepackage[UTF8]{ctex}
\begin{table*}[htbp]
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{c|c|c|cccccc}
\toprule

\multirow{2}{*}{train\_size=1000} &
  \multirow{2}{*}{\textbf{aspect}} &
  \multirow{2}{*}{\textbf{未提及数量}} &
  \multicolumn{6}{c}{\textbf{$\Delta$ Kappa}} \\
 & & & \textbf{LLaMA-Chat} &
  \textbf{LLaMA-Base} &
  \textbf{InternLM-Chat} &
  \textbf{InternLM-Base} &
  \textbf{Baichuan2-Chat} &
  \textbf{Baichuan2-Base} \\
\hline

D1 & 食品评价   & 131   & -1.21\% & -0.27\%  & 0.90\%   & -0.91\%  & -0.48\%  & 0.84\%   \\
   & 价格水平   & 3,120 & -1.19\% & -1.70\%  & -0.77\%  & -2.18\%  & -0.07\%  & -3.76\%  \\
   & 服务人员态度 & 3,183 & -0.46\% & -0.68\%  & -1.09\%  & -0.79\%  & -0.30\%  & -4.88\%  \\
   & 饮品评价   & 5504  & -2.11\% & -1.17\%  & -0.08\%  & 0.70\%   & -1.32\%  & -1.89\%  \\
   & 卫生情况   & 6,174 & 0.52\%  & 0.39\%   & -0.16\%  & -1.80\%  & -1.34\%  & -4.81\%  \\
   & 停车方便程度 & 7,505 & -1.58\% & 2.22\%   & -1.57\%  & -6.03\%  & -2.27\%  & -5.34\%  \\
\hline

D2 & 交通便利程度 & 2,516 & -0.40\% & 0.21\%   & -9.84\%  & -4.29\%  & -4.68\%  & -10.68\% \\
   & 装修情况   & 3,501 & -0.47\% & -2.95\%  & -2.44\%  & -8.49\%  & -5.49\%  & -3.57\%  \\
   & 排队等候情况 & 5,171 & 0.63\%  & 1.03\%   & -5.31\%  & -4.02\%  & -6.14\%  & -1.47\%  \\
   & 点菜上菜速度 & 5,850 & 0.28\%  & -7.36\%  & -5.68\%  & -11.40\% & -11.81\% & -8.11\%  \\
   & 嘈杂情况   & 7,448 & 6.58\%  & -19.97\% & -11.03\% & -16.21\% & -10.36\% & -5.97\%  \\
\bottomrule      
\end{tabular}
\end{table*}
%\end{CJK*}

==> tables/mentioned-only_500.tex <==
%-- coding: UTF-8 --
%\usepackage{CJKutf8}
%\begin{CJK*}{UTF8}{gbsn}

\begin{table*}[htbp]
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{c|c|c|cccccc}

\toprule
\multirow{2}{*}{train\_size=500} &
  \multirow{2}{*}{\textbf{aspect}} &
  \multirow{2}{*}{\textbf{未提及数量}} &
  \multicolumn{6}{c}{\textbf{$\Delta$ Kappa}} \\
 & & & \textbf{LLaMA-Chat} &
  \textbf{LLaMA-Base} &
  \textbf{InternLM-Chat} &
  \textbf{InternLM-Base} &
  \textbf{Baichuan2-Chat} &
  \textbf{Baichuan2-Base} \\
\hline

D1 & 食品评价   & 131   & -0.95\%  & -0.86\%  & 1.09\%   & 0.46\%   & -0.26\%  & 0.60\%   \\
   & 服务人员态度 & 3,120 & -0.63\%  & -3.27\%  & -2.41\%  & -6.22\%  & -11.03\% & -5.35\%  \\
   & 卫生情况   & 3,183 & -1.66\%  & -3.98\%  & -5.53\%  & -9.78\%  & -13.42\% & -2.88\%  \\
   & 价格水平   & 5504  & -2.82\%  & -3.55\%  & 0.72\%   & -0.87\%  & -10.30\% & -4.32\%  \\
   & 饮品评价   & 6,174 & -0.35\%  & -2.98\%  & -8.87\%  & -17.62\% & -18.53\% & -20.40\% \\
   & 停车方便程度 & 7,505 & -15.72\% & -26.05\% & -14.83\% & -39.55\% & -39.60\% & -12.11\% \\
\hline

D2 & 交通便利程度 & 2,516 & -3.28\%  & -15.38\% & -18.09\% & -3.45\%  & -5.37\%  & -21.41\% \\
   & 点菜上菜速度 & 3,501 & -9.98\%  & -38.91\% & -12.58\% & -26.05\% & -10.63\% & -9.30\%  \\
   & 装修情况   & 5,171 & -3.82\%  & -7.37\%  & -7.06\%  & -4.44\%  & 1.02\%   & -5.82\%  \\
   & 排队等候情况 & 5,850 & -20.76\% & -26.25\% & -29.59\% & -27.17\% & -25.76\% & -23.82\% \\
   & 嘈杂情况   & 7,448 & -36.54\% & -47.60\% & -30.66\% & -35.76\% & -33.22\% & -35.25\% \\
 
\bottomrule    


\end{tabular}
\end{table*}
%\end{CJK*}

==> tables/perplexity.tex <==
\begin{table}[h]
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lccc}
\toprule[1.2pt]
& LLaMA2-Chat &InternLM-Chat &Baichuan2-Chat\\
\hline

Ins-last  & 1.524      & 1.631         & 1.803    \\
Ins-first & 1.546      & 2.016         & 1.961    \\
T2T       & 18.623     & 30.639        & 31.226   \\
\hline
Natural   & 1.524      & 1.631         & 1.803    \\
Lines     & 1.538      & 1.705         & 2.051    \\
Dict      & 1.185      & 1.323         & 1.345    \\
Numerical & 1.666      & 2.040         & 2.174    \\
MO        & 3.153      & 4.077         & 8.207    \\
\hline
No-CoT    & 1.185      & 1.323         & 1.345    \\
CoT       & 1.349      & 1.442         & 1.406    \\
Rev-CoT   & 1.346      & 1.453         & 1.430    \\

\midrule[1.2pt]

&LLaMA2-Base &InternLM-Base &Baichuan2-Base\\
\hline

Ins-last  & 1.913      & 2.138         & 2.035    \\
Ins-first & 1.980      & 1.899         & 1.733    \\
T2T       &            & 25.119        & 25.566   \\
\hline
Natural   & 1.913      & 2.138         & 2.035    \\
Lines     &            & 2.163         & 2.142    \\
Dict      & 4.970      & 1.562         & 1.344    \\
Numerical & 2.012      & 2.336         & 2.089    \\
MO        & 13.806     & 6.037         & 5.996    \\
\hline
No-CoT    & 4.970      & 1.562         & 1.344    \\
CoT       & 2.819      & 1.499         & 1.397    \\
Rev-CoT   & 3.004      & 1.559         & 1.418 \\
\bottomrule[1.2pt]
\end{tabular}
\caption{Perplexity analysis.}
\label{fig:perplexity_old}
\end{table}
